On the generalization of learned constraints for ASP solving in temporal domains

The representation of a dynamic problem in ASP usually boils down to using copies of variables and constraints, one for each time stamp, no matter whether it is directly encoded or via an action or temporal language. The multiplication of variables and constraints is commonly done during grounding and the solver is completely ignorant about the temporal relationship among the different instances. On the other hand, a key factor in the performance of today's ASP solvers is conflict-driven constraint learning. Our question is now whether a constraint learned for particular time steps can be generalized and reused at other time stamps, and ultimately whether this enhances the overall solver performance on temporal problems. Knowing full well the domain of time, we study conditions under which learned dynamic constraints can be generalized. We propose a simple translation of the original logic program such that, for the translated programs, the learned constraints can be generalized to other time points. Additionally, we identify a property of temporal problems that allows us to generalize all learned constraints to all time steps. It turns out that this property is satisfied by many planning problems. Finally, we empirically evaluate the impact of adding the generalized constraints to an ASP solver. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> Makefile <==
all: init
	latexmk paper.tex -pdf

watch: init
	latexmk paper.tex -pdf -pvc

clean:
	latexmk paper.tex -pdf -C

init: .initialized

SHELL=bash
.initialized:
	test ! -d .git || git config -f .gitmodules --get-regexp '^submodule\..*\.path$$' | \
	  while read path_key path_val; do \
	    url_key=$$(echo $$path_key | sed 's/\.path/.url/'); \
	    url=$$(git config -f .gitmodules --get "$$url_key"); \
	    git submodule add $$url $$path_val || true; \
	    git submodule update --init --recursive $$path_val; \
	  done
	touch .initialized

.PHONY: all watch clean init


==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

\begin{itemize}
\item Patrick (ICLP)
\item Taupe, Weinzierl (LPNMR'19??)
\item Scheuller (IJCAI)
\end{itemize}

\url{potassco.org}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/dtel.tex <==
\RequirePackage{bm}
\RequirePackage{textcomp}
\RequirePackage{upgreek}

\IfFileExists{outline.tex}{\input{outline}}{}

\newcommand{\next}{\text{\rm \raisebox{-.5pt}{\Large\textopenbullet}}}  % {{\ensuremath{\circ}}}
\newcommand{\previous}{\text{\rm \raisebox{-.5pt}{\Large\textbullet}}}  % {{\ensuremath{\bullet}}}
\newcommand{\wnext}{\ensuremath{\widehat{\next}}}
\newcommand{\wprevious}{\ensuremath{\widehat{\previous}}}
\newcommand{\alwaysF}{\ensuremath{\square}}
\newcommand{\alwaysP}{\ensuremath{\blacksquare}}
\newcommand{\eventuallyF}{\ensuremath{\Diamond}}
\newcommand{\eventuallyP}{\ensuremath{\blacklozenge}}
\IfFileExists{outline.tex}
        {\newcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}}
        {\newcommand{\until}{\ensuremath{\mathbin{\bm{\mathsf{U}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}}
        {\newcommand{\release}{\ensuremath{\mathbin{\bm{\mathsf{R}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\while}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{W}}$}}}}}}
        {\newcommand{\while}{\ensuremath{\mathbin{\bm{\mathsf{W}}}}}}
\newcommand{\since}{\ensuremath{\mathbin{\bm{\mathsf{S}}}}}
\newcommand{\trigger}{\ensuremath{\mathbin{\bm{\mathsf{T}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}}
        {\newcommand{\finally}{\ensuremath{\bm{\mathsf{F}}}}}
\newcommand{\initially}{\ensuremath{\bm{\mathsf{I}}}}

\newcommand{\stp}{\ensuremath{\uptau}}

\newcommand{\dalways}[1]{\ensuremath{[#1]\,}}                        % \DBox
\newcommand{\deventually}[1]{\ensuremath{\langle#1\rangle\,}}        % \DDia
\newcommand{\drel}[2]{\ensuremath{{\parallel}{#1}{\parallel}^{#2}}}  % \Rel

\newcommand{\intervcc}[2]{\ensuremath{[#1..#2]}}
\newcommand{\intervco}[2]{\ensuremath{[#1..#2)}}
\newcommand{\intervoc}[2]{\ensuremath{(#1..#2]}}
\newcommand{\intervoo}[2]{\ensuremath{(#1..#2)}}
\newcommand{\rangecc}[3]{\ensuremath{#1 \in \intervcc{#2}{#3}}}
\newcommand{\rangeco}[3]{\ensuremath{#1 \in \intervco{#2}{#3}}}
\newcommand{\rangeoc}[3]{\ensuremath{#1 \in \intervoc{#2}{#3}}}
\newcommand{\rangeoo}[3]{\ensuremath{#1 \in \intervoo{#2}{#3}}}


==> include/asp-macros/grounding.tex <==
\newcommand{\ground}[1]{\ensuremath{\mathit{ground}(#1)}}
\newcommand{\cground}[2]{\ensuremath{\mathit{ground}_{#2}(#1)}}

\newcommand{\vars}[1]{\mathit{vars}(#1)}
\newcommand{\match}[2]{\mathit{match}_{#2}(#1)}


==> include/asp-macros/ht.tex <==

\newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\Htrace}{\ensuremath{\mathbf{H}}}
\newcommand{\Ttrace}{\ensuremath{\mathbf{T}}}
\newcommand{\M}{\ensuremath{\mathbf{M}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> include/asp-macros/listings.tex <==
% The language definitions below require the following packages:
%
%     \usepackage{courier}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%     \renewcommand{\Underscore}{\textscale{1}{\textunderscore}}
%
% Without extra packages I had to provide an alternative underscore definition
% to get decent looking underscores.
%
% As an alternative to courier, it is also possible to use the `lmodern`
% package.
%
%     \usepackage[T1]{fontenc}
%     \usepackage{lmodern}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%
% When the python or clingo language is given, tex code can be embedded
% escaping it in `#( ... #)`, which is treated like a comment in Python.
% Furthermore, for logic programs the character sequence is `%%` is not output.
% This can be used to add labels at the end of lines. For example, in a logic
% program one can write
%
%     H :- B.%%#( \label{lst:rule} #)
%
% to refer to the rule from the document without having to worry about changing
% line numbers when refactoring. The annotated program will still be runnable
% with clingo.

\providecommand{\Underscore}{\textunderscore}

\lstdefinelanguage{clingo}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  keywordstyle=[2]\bfseries,%
  keywordstyle=[3]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}1 {\%\%}{}0,%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  keywords=[2]{\#const,\#show,\#minimize,\#base,\#theory,\#count,\#external,\#program,\#script,\#end,\#heuristic,\#edge,\#project,\#show,\#sum},%
  keywords=[3]{&,&dom,&sum,&diff,&show},%
  morecomment=[l]{\#\ },%
  morecomment=[l]{\%\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}

\lstdefinelanguage{python}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}{1},%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  morecomment=[l]{\#\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}



==> include/asp-macros/logics.tex <==
\providecommand{\logfont}{\textrm}

\newcommand{\HT}{\ensuremath{\logfont{HT}}}
\newcommand{\EL}{\ensuremath{\logfont{EL}}}

\newcommand{\HTC}{\ensuremath{\logfont{HT}_{\!c}}}

\newcommand{\LTL}{\ensuremath{\logfont{LTL}}}
\newcommand{\LTLf}{\ensuremath{\LTL_{\!f}}}
\newcommand{\LTLo}{\ensuremath{\LTL_{\omega}}}
\newcommand{\THT}{\ensuremath{\logfont{THT}}}
\newcommand{\THTf}{\ensuremath{\THT_{\!f}}}
\newcommand{\THTo}{\ensuremath{\THT_{\!\omega}}}
\newcommand{\TEL}{\ensuremath{\logfont{TEL}}}
\newcommand{\TELf}{\ensuremath{\TEL_{\!f}}}
\newcommand{\TELo}{\ensuremath{\TEL_{\omega}}}
%
\newcommand{\LDL}{\ensuremath{\logfont{LDL}}}
\newcommand{\LDLf}{\ensuremath{\LDL_{\!f}}}
\newcommand{\LDLo}{\ensuremath{\LDL_{\omega}}}
\newcommand{\DHT}{\ensuremath{\logfont{DHT}}}
\newcommand{\DHTf}{\ensuremath{\DHT_{\!f}}}
\newcommand{\DHTo}{\ensuremath{\DHT_{\!\omega}}}
\newcommand{\DEL}{\ensuremath{\logfont{DEL}}}
\newcommand{\DELf}{\ensuremath{\DEL_{\!f}}}
\newcommand{\DELo}{\ensuremath{\DEL_{\omega}}}
%
\newcommand{\DL}{\ensuremath{\logfont{DL}}}

\newcommand{\MTL}{\ensuremath{\logfont{MTL}}}
\newcommand{\MTLf}{\ensuremath{\MTL_{\!f}}}
\newcommand{\MTLo}{\ensuremath{\MTL_{\omega}}}
\newcommand{\MHT}{\ensuremath{\logfont{MHT}}}
\newcommand{\MHTf}{\ensuremath{\MHT_{\!f}}}
\newcommand{\MHTo}{\ensuremath{\MHT_{\!\omega}}}
\newcommand{\MEL}{\ensuremath{\logfont{MEL}}}
\newcommand{\MELf}{\ensuremath{\MEL_{\!f}}}
\newcommand{\MELo}{\ensuremath{\MEL_{\omega}}}


==> include/asp-macros/modules.tex <==
% - modules ----------------------------------------
\newcommand{\module}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\prog}[1]{\ensuremath{P(#1)}}
\newcommand{\inp}[1]{\ensuremath{I(#1)}}
\newcommand{\out}[1]{\ensuremath{O(#1)}}
\newcommand{\inst}[2]{\ensuremath{#1(#2)}}
% \newcommand{\exts}{\epsilon}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> include/asp-macros/nogoods.tex <==
\newcommand{\domain}[1]{\ensuremath{\mathit{dom}(#1)}}

\newcommand{\ass}{\ensuremath{A}}

\newcommand{\tlits}[1]{\ensuremath{{#1}^{\true}}}
\newcommand{\flits}[1]{\ensuremath{{#1}^{\false}}}
\newcommand{\prefix}[2]{\ensuremath{#1[#2]}}

\newcommand{\clno}[1]{\ensuremath{\delta(#1)}}
\newcommand{\ClNo}[1]{\ensuremath{\Delta(#1)}}
% \newcommand{\nocl}[1]{\ensuremath{\gamma(#1)}}
% \newcommand{\NoCl}[1]{\ensuremath{\Gamma(#1)}}

\newcommand{\CN}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\LN}[1]{\ensuremath{\Lambda_{#1}}}

\newcommand{\dl}[0]{\ensuremath{\mathit{dl}}}
\newcommand{\dlevel}[1]{\ensuremath{\mathit{dlevel}(#1)}}
\newcommand{\opp}[1]{\ensuremath{\overline{#1}}}

% \newcommand{\undef}[0]{\ensuremath{\circ}}
% \newcommand{\trdef}[0]{\ensuremath{\times}}
\newcommand{\scc}[1]{\ensuremath{\mathit{scc}(#1)}}
\newcommand{\source}[1]{\ensuremath{\mathit{source}(#1)}}


==> include/asp-macros/operators.tex <==

% - operators ------------------------------------------------------------------

\newcommand{\Top}[1]{\ensuremath{T_{#1}}}
\newcommand{\T}[2]{\Top{#1}#2}
\newcommand{\Topi}[2]{\Top{#2}^{#1}}
\newcommand{\Ti}[3]{\Topi{#1}{#2}#3}

% - semantic operators -----------------------------------------------------------

\newcommand{\SM}[1]{\ensuremath{\mathit{SM}(#1)}}


==> include/asp-macros/outline.tex <==
\RequirePackage{xcolor}
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/tableau.tex <==

\newcommand{\Tsigned}[1]{\ensuremath{\true{#1}}}\message{ *** RENAME, Tlit,Flit ?? *** }
\newcommand{\Fsigned}[1]{\ensuremath{\false{#1}}}

\newcommand{\TOP}[1]{\ensuremath{D_{#1}}}
\newcommand{\COP}[1]{\ensuremath{D^*_{#1}}}

\newcommand{\Proviso}[1]{\raisebox{-7pt}[0pt][0pt]{\ensuremath{(#1)}}}

\newcommand{\plit}[1]{\ensuremath{\boldsymbol{t}{#1}}}
\newcommand{\nlit}[1]{\ensuremath{\boldsymbol{f}{#1}}}


==> instance.tex <==
\section{Blocks World problem instance}\label{sec:instance}

This is the full ASP code of the instance of our example.

\lstset{style=appendixstyle}

\begin{lstlisting}%
%
% instance
%

block(a;b;c).  init(clear(a)). init(handempty).
init(on(a,b)). init(on(b,c)). init(ontable(c)).
goal(on(b,a)). goal(on(c,b)). goal(ontable(a)).


%
% actions
%

action(pick_up(X))         :- block(X).
pre(pick_up(X),  clear(X)) :- block(X).
pre(pick_up(X),ontable(X)) :- block(X).
pre(pick_up(X), handempty) :- block(X).
add(pick_up(X),holding(X)) :- block(X).
del(pick_up(X),ontable(X)) :- block(X).
del(pick_up(X),  clear(X)) :- block(X).
del(pick_up(X), handemtpy) :- block(X).

action(put_down(X))         :- block(X).
pre(put_down(X),holding(X)) :- block(X).
add(put_down(X),  clear(X)) :- block(X).
add(put_down(X), handempty) :- block(X).
add(put_down(X),ontable(X)) :- block(X).
del(put_down(X),holding(X)) :- block(X).

action(stack(X,Y))         :- block(X), block(Y).
pre(stack(X,Y),holding(X)) :- block(X), block(Y).
pre(stack(X,Y),  clear(Y)) :- block(X), block(Y).
del(stack(X,Y),holding(X)) :- block(X), block(Y).
del(stack(X,Y),  clear(Y)) :- block(X), block(Y).
add(stack(X,Y),  clear(X)) :- block(X), block(Y).
add(stack(X,Y), handempty) :- block(X), block(Y).
add(stack(X,Y),   on(X,Y)) :- block(X), block(Y).

action(unstack(X,Y))       :- block(X), block(Y).
pre(unstack(X,Y),   on(X,Y)) :- block(X), block(Y).
pre(unstack(X,Y),  clear(X)) :- block(X), block(Y).
pre(unstack(X,Y), handempty) :- block(X), block(Y).
add(unstack(X,Y),holding(X)) :- block(X), block(Y).
add(unstack(X,Y),  clear(Y)) :- block(X), block(Y).
del(unstack(X,Y),  clear(X)) :- block(X), block(Y).
del(unstack(X,Y), handempty) :- block(X), block(Y).
del(unstack(X,Y),   on(X,Y)) :- block(X), block(Y).
\end{lstlisting}



==> pitwo.tex <==
\section{Program $\Pi_2$ from Example~\ref{example:cyclic:one}}
\label{appendix:program}

This is the program $\Pi_2$ from Example~\ref{example:cyclic:one}.



==> semantics.tex <==
\newcommand{\true}{\ensuremath{\boldsymbol{T}}}
\newcommand{\false}{\ensuremath{\boldsymbol{F}}}

\newcommand{\Cn}[1]{\ensuremath{\mathit{Cn}(#1)}}
\newcommand{\reduct}[2]{\ensuremath{#1^{#2}}}

\newcommand{\Loops}[1]{\ensuremath{\mathit{Loop}(#1)}}

% - formulas ---------------------------------------------------------------------

\newcommand{\BF}[1]{\ensuremath{\mathit{BF}(#1)}}
\newcommand{\CF}[1]{\ensuremath{\mathit{CF}(#1)}}
\newcommand{\LF}[1]{\ensuremath{\mathit{LF}(#1)}}

\newcommand{\CFIF}[1]{\ensuremath{\overleftarrow{\mathit{CF}}(#1)}}
\newcommand{\CFFI}[1]{\ensuremath{\overrightarrow{\mathit{CF}}(#1)}}
\newcommand{\CFX}[1]{\ensuremath{\mathit{CF}^x(#1)}}

\newcommand{\ES}[2]{\ensuremath{\mathit{ES}_{\!#2}(#1)}}
\newcommand{\EB}[2]{\ensuremath{\mathit{EB}_{\!#2}(#1)}}
\newcommand{\LFS}[2]{\ensuremath{\mathit{LF}_{\!#2}(#1)}}

==> tempnogoods.tex <==
%\section{Solving temporal logic problems}\label{sec:tempnogoods}
\begin{itemize}

% --------------------------------------------------------------------------------
\item
Completion nogoods characterize answer sets of the generator program
whenever it is tight.
%
% ------------------------------------------------------------
\begin{proposition}\label{thm:nogoods:tight:temp}
Let $\Pi$ be a tight temporal logic program
and 
% let $\Delta_\Pi$ be the set of nogoods
\[
\begin{array}{@{}l@{}c@{}l}
\Delta_\Pi & {} = {} &
\{\clno{\beta} \mid \beta\in\body{{\Pi}\setminus\integr{\Pi}}\} 
\cup
\{\delta\in\ClNo{\beta}\mid \beta\in\body{{\Pi}\setminus{\integr{\Pi}}}\} 
\\[2pt]
& \cup &
\{\clno{p} \mid p\in\mathcal{P}\}
\cup
\{\delta\in\ClNo{p} \mid p\in\mathcal{P}\}
\\[2pt]
& \cup &
\{\clno{\beta}\setminus\{\Flit\beta\} \mid \beta\in\body{\integr{\Pi}}\}.
\end{array}
\]
%
Then, 
$X\subseteq\atom{\Pi}$ is an answer set of~$\Pi_g$
iff
$X=\Tass{A}\cap\atom{\Pi}$ for a (unique) 
solution $A$ for $\Delta_\Pi$.
\end{proposition}
% ------------------------------------------------------------
%
Observe that the atoms $p \in \mathcal{P}'$ are left open simply 
by not adding their corresponding atom-oriented nogoods $\clno{p}$ and $\delta\in\ClNo{p}$.

% --------------------------------------------------------------------------------
\item
We get the following set of loop nogoods for a temporal logic program $\Pi$\/:
\begin{equation}
\begin{array}{l@{}l}
  \label{eq:ub:nomore:temp}
  \Lambda_\Pi
  = {} &
  \mbox{$\bigcup_{U\subseteq \mathcal{P},U\neq\emptyset}$}
  \{ 
%    (\Flit{\beta_1},\dots,\Flit{\beta_k},\Tlit{p}) 
\lambda(p,U)
  \mid 
%  {} \\[1mm] & \qquad\qquad
%    \EB{U}{\Pi}=\{\beta_1,\dots,\beta_k\},
    p\in U
  \}
\end{array}
\end{equation}
Similar to before, for the loop nogoods we do not consider the atoms $p \in \mathcal{P}'$.

% --------------------------------------------------------------------------------
\item
Completion and loop nogoods characterize answer sets of the generator program in general.
%
If $\Pi$ is a temporal logic program,
by $\Sigma_\Pi$ we denote the set
of completion and loop nogoods of the generator program $\Delta_\Pi \cup \Lambda_\Pi$
where $\Delta_\Pi$ and $\Lambda_\Pi$ % be 
are as in Theorem~\ref{thm:nogoods:tight:temp} and~(\ref{eq:ub:nomore:temp}), respectively.
%
% ------------------------------------------------------------
\begin{proposition}\label{thm:nogoods:nontight:temp}
Let $\Pi$ be a temporal logic program.
%% and
%let 
%$\Delta_\Pi$ and $\Lambda_\Pi$ % be 
%as % given 
%in Theorem~\ref{thm:nogoods:tight:temp} and~(\ref{eq:ub:nomore:temp}).%
%\SPACY{}
Then, 
$X\subseteq\atom{\Pi}$ is an answer set of~$\Pi_g$
iff
$X=\Tass{A}\cap\atom{\Pi}$ for a (unique)
%solution $A$ for $\Delta_\Pi\cup\Lambda_\Pi$.
solution $A$ for $\Sigma_\Pi$.
\end{proposition}
% ------------------------------------------------------------
%

% --------------------------------------------------------------------------------
\item
They are easily extended to characterize solutions of temporal logic problems.

\begin{theorem}\label{thm:nogoods:temporal}
Let \tpb{\Pi}{I}{F} be a temporal logic problem. 
%and  
%let 
%$\Delta_\Pi$ and $\Lambda_\Pi$  be 
%as % given 
%in Theorem~\ref{thm:nogoods:tight:temp} and~(\ref{eq:ub:nomore:temp}).%
%\SPACY{}
%
The pair $(n,X)$ is a solution to \tpb{\Pi}{I}{F}
for some integer $n\geq 1$ and 
$X\subseteq\btw{\mathcal{P}}{0}{n}$ 
iff
$X=\Tass{A}\cap\btw{\mathcal{P}}{0}{n}$ for a (unique)
solution $A$
%for $\btw{(\Delta_\Pi\cup\Lambda_\Pi)}{1}{n}$
for $\btw{\Sigma_\Pi}{1}{n}$
such that $(\at{I}{0} \cup \at{F}{n}) \subseteq A$.
\end{theorem}

Observe that we have $n$ copies of the nogoods for the generator program, 
and \emph{nothing else}.

\item
Solving: scheduler selects values of $n$ to look for solutions $(n,X)$.
%
For each $n$, it calls 

\end{itemize}

